Variable-Scaling Rate Control for Collision-Free Teleoperation of an Unmanned Aerial Vehicle

We propose that automatically adjusting the scale factor in rate-control teleoperation could enable a human operator to better control the motion of a remote robot. In this paper, we present four new variable-scaling rate-control methods that adjust the scale factor depending on the state of the user's input commands and/or the risk of a collision between the robot and its environment. Methods that depend on the risk of a collision are designed to guarantee collision avoidance by setting the scale factor to be zero if the operator issues a command that would result in a collision between the robot and its environment. A within-subject user study was conducted to determine the effects of the four newly designed rate-control methods and a traditional fixed-scale rate-control method on a person's ability to complete a navigation task in a simulated two-dimensional environment. The results of this study indicate that well-designed variable-scale rate control can guarantee collision-free teleoperation without reducing task efficiency.

==> scrap.tex <==
where $S_{risk}$ is calculated from Equation \ref{eq:maxcrp}.

$$
S = S_c*min(1, \frac{P_{input}}{P_c} )\eqno{(8)} 
$$

\item Considering the highest risk of collision $C_r$. which will happen in X-axis direction in our reference frame, this method can be explained as follows:

$$
S = S_c*(1-C_r)*min(1, \frac{P_{input}}{P_c} )\eqno{(9)} 
$$

\item Calculating the risk of collision in X-axis and Y-axis without considering the direction of the UAV's velocity, two risks of collision, $C_{rx}$ and $C_{ry}$, will be generated. The mapping scales are described by
$$
S_x = S_c*(1-C_{rx})*min(1, \frac{P_{input}}{P_c} )\eqno{(10)} 
$$
$$
S_y = S_c*(1-C_{ry})*min(1, \frac{P_{input}}{P_c} )\eqno{(11)} 
$$
where $S_x$ and $S_y$ are the mapping scale in the reference frame that we defined.
\item Calculating the risk of collision in X-axis and Y-axis by considering the direction of the UAV's velocity, four risks of collision will be generated. Then the mapping scales can be calculated by
$$
S_{x}=\left\{\begin{matrix}S_c*(1-C_{rpx})*min(1, \frac{P_{input}}{P_c} ), &\vec{v}\cdot \vec{x} \geq 0\ \\
 S_c*(1-C_{rnx})*min(1, \frac{P_{input}}{P_c} ),& \vec{v}\cdot \vec{x} < 0\
\end{matrix}\right.\eqno{(12)} 
$$
$$
S_{y}=\left\{\begin{matrix}S_c*(1-C_{rpy})*min(1, \frac{P_{input}}{P_c} ), &\vec{v}\cdot \vec{y} \geq 0\ \\
 S_c*(1-C_{rny})*min(1, \frac{P_{input}}{P_c} ),&\vec{v}\cdot \vec{y} < 0\
\end{matrix}\right.\eqno{(13)} 
$$
where $C_{rpx}$, $C_{rnx}$, $C_{rpy}$ and  $C_{rny}$ are the risks of collision in positive $X$, negative $X$, positive $Y$ and negative $Y$ directions. $\vec{v}$ is the unit vector of the UAV's velocity, $\vec{x}$ is the unit vector pointing to positive X-axis direction, and $\vec{y}$ is the unit vector pointing to positive Y-axis direction.



Correspondingly, we designed five methods to generate the mapping scale in rate control, one for constant mapping scale and four for variable mapping scale.


\subsubsection{Constant Mapping Scale}

A constant scale was mostly used in traditional rate-control method, which means the mapping scale $S$ is a predefined constant value, $S_c$, as described by $S$ = $S_{c}$.

\subsubsection{Variable Mapping Scale}






%\textcolor{red}{if we need to clarify how to rotate from global frame to reference frame and how to rotate back?}
In the variable mapping method, the mapping scales are generated in local reference frame, and both of the user's input and the command for the UAV's velocity are in the global frame. When implementing the method, the user's input needs to be translated to be in local frame, then the obtained command for UAV's velocity needs to be translated back to the global frame. All the translating calculation is realized by rotation matrices which are generated by the angles between the local frame and the global frame.


\subsection{Collision Avoidance}

In the variable mapping scale method, we are changing the mapping scale between the user's the input and the commands sent to command the remote UAV based on the user's input and a risk of collision. If the UAV flies towards to or extremely close to obstacles, a risk of collision will approach to a value of 1, while the mapping scale in the direction where the highest risk of collision may happen will decrease almost to a value of 0, making the velocity command send to the UAV also approach to a value of 0. Theoretically, the UAV will stop before colliding with obstacles. Also, the PRF, the method we applied to generate the risk of collision, gives the UAV enough time to decelerate before the collision happens.





There is one goal location in the free space close to the starting location, two target locations in the corner of the 

A informed consent form was given to each subject before starting the study. 
At the beginning of the study, the goal of each task was explained to each subject, which is to move the virtual UAV from a starting position to three objects sequentially. In this process, they were required to finish as soon as possible and also required to avoid colliding with the obstacle in the environment.

At the end of each task, subjects were asked to rate the difficulty of the task by completing a NASA Task Load Index (NASA-TLX) \cite{hart1988}.

At the end of the study, each of the subject completed a survey to provide the preference of the methods against different requirements of the task. 






 \begin{figure}[t] 
      \centering

      \includegraphics[width=\columnwidth,clip]{trialTimes.eps}
      \caption{\small  A Logitech EXTREME 3D Pro joystick that is used as the control interface in the user study}
      \label{fig:resultsTrialTimes}
      \vspace{-10pt}
   \end{figure}
   
     \begin{figure}[t] 
      \centering

      \includegraphics[width=\columnwidth,clip]{distanceTraveled.eps}
      \caption{\small  A Logitech EXTREME 3D Pro joystick that is used as the control interface in the user study}
      \label{fig:resultsDistance}
      \vspace{-15pt}
   \end{figure}
   
   
        \begin{figure}[t] 
      \centering

      \includegraphics[width=\columnwidth,clip]{collisionTime.eps}
      \caption{\small  A Logitech EXTREME 3D Pro joystick that is used as the control interface in the user study}
      \label{fig:resultsCollision}
      \vspace{-15pt}
   \end{figure}
   
          \begin{figure}[t] 
      \centering

      \includegraphics[width=\columnwidth,clip]{overshoot.eps}
      \caption{\small  A Logitech EXTREME 3D Pro joystick that is used as the control interface in the user study}
      \label{fig:resultsCollision}
      \vspace{-15pt}
   \end{figure}
   
   
   
   

   
   
   
   \subsubsection{$T_{task}$}
As shown in Fig. 5 (a) there is significant difference in $T_{task}$ when comparing method R1 with the other four methods, which means the users spent more time to complete the task when applying method R1. In addition, the P value of method R2 and R3 is 0.004, indicating that there is also significant difference in $T_{task}$ between R2 and R3.
\subsubsection{$D_{total}$}
In general, there is no significant difference in $D_{total}$ among method C,H,R1 and R3. However, when comparing method R2 with method H, R1 and R3, a significant difference can be observed, and $D_{total}$ for method R2 is obviously greater than $D_{total}$ obtained from other three methods.
\subsubsection{$T_{collision}$}

From the results shown in Fig. 5(c), we can see that no collisions with the virtual wall happened when applying methods R1, R2 and R3, while collisions happened when applying methods C and method H. The P value between method C and method H is greater than 0.05, we can't conclude that there is obvious difference in $T_{collision}$ between method C and method H.
\subsubsection{$D_{overshoot}$}
As we can see from Fig. 5(d), the overshoot happened mostly when applying method R1, R2 and R3. In addition, the $D_{overshoot}$ obtained from method R3 is relatively smaller than the $D_{overshoot}$ obtained from method R1. The P value is 1.161e-13 , indicating the difference is significant.


 
 
 
 
 -travel time: (F(4,56) =99.825, p = 8.4032e-25)
-travel distance: (F(4,56) =8.5167, p = 1.93e-05)
-collision time, ttest, p = 4261. 
-overshoot F(4,56) = 31.166   p = 1.161e-13 
F(2,28) =  26.183    p = 3.8832e-07





The results of this study indicate that variable-scaling rate control can improve a person's ability to control a UAV. Importantly, we note that by taking into account the risk that the robot will collide with its environment, variable-scaling rate control can guarantee that the human operator will not crash the remote robot. Calculating a single scale factor based on the overall highest risk of a collision, as is done in Method R1, reduces the speed at which the operator can fly the UAV in constrained areas. The is reflected by the increased time it took the operators to complete the task when using Method R1. Calculating separate scale factors for the direction pointing to the object in the UAV's environment posing the biggest collision risk and a direction perpendicular to this, as is done in R2, can significantly increase the speed with which the user can fly the UAV. This is especially true for a hallway scenario, where the distance between the UAV and a wall will typically be much smaller than the distance between the UAV an object along the length of hallway. Moreover, calculating separate scale factors for two perpendicular directions accounting only for the risk of collision with objects in the direction of the commanded velocity, as is done in Method R3, resulted in faster task completion times than considering the overall all risk in these directions. Notably, the results of the user study indicated that Method R3 did not effect the user's task completion time, as compared to method that did not slow the UAV down when the risk of a collision was high. The finding that Method R3 did not result in decrease task efficiency is also reflected in the fact that nearly as many study participants indicated that they most prefer to complete a task quickly using this method, as compared to the number of participants who selected the method that never reduced the scale factor. 

One limitation of reducing the scale factor when the risk of collision is high, is that our results indicate that it may be difficult to people to control the position of the robot when the risk of collision transitions from high to low. In this study, under Method R1, R2, and R3, when the UAV exited the hallway, the same position of the joystick will suddenly result in higher commanded speed to the robot. Nearly all participants overshot the target located near the hallway's exit under Methods R1 and R2, and about half of the participants overshot this target when using Method R3. Only three participants overshot this target when using the conditions that did not reduce the scale factor based on the risk of a collision between the UAV and an object in its environment. This indicates that there should be limits on the rate with which the overall rate-control scale factor can be increased. 

There are no difference between user performance when using the rate-control method that reduced the scale factor based on the user's input, H, and the user performance when using the rate-control method that never reduced the scale factor, C. However, participants were still likely to be able to perceive a difference between these conditions, as indicated by the fact that seven of the fifteen participants indicated that they would most prefer to use Method C to complete a task quickly, while not participants indicated that they would most prefer to used Method H. 


Based on the results of the user study, method R3, which adjusts the rate-control's scale factor based on user's input, risk of collision in the X- and Y- direction accounting only for the risk of collision with objects in the direction of the commanded velocity, has a best overall performance. 
 
 
 
 
 %From the results of $T_{trial}$, we can see that method R1 took more time to complete the task compared with other methods. We believe it is because in method R1, the scale factor in all direction is based on the highest risk of collision. When the UAV was moved closely to the obstacles, scale factor were kept as the smallest value in all directions, which slowed down the commanded velocity. We believe this is also the reason why the users chose method R1 as their least favorite method if they were asked to finish the task quickly. Both method R2 and method R3 had better performance than method R1 in $T_{trial}$, it is because the scale factor in method R2 and method R3 is based on the risk of collision in different directions. Also, method R3 has better performance than method R2 and nearly has the same $T_{trial}$ with method C and H, which indicates that considering the direction of the commanded velocity in generating scale factor can improve the speed performance of the UAV, even though the UAV's speed will be slowed down when getting close to the obstacles.

%The only significant difference in $D_{total}$ is that method R2 has more traveled distance than other methods. This is in line with the results of $D_{overshoot}$, which indicates that the users had more overshoot when under method R2 than under other methods. We believe these results can be explained by the difficulty for the user to get used to the increased scale when the UAV moved out from the constrained hallway.Especially for methods R2, the rate-control without considering the directions of the commanded velocity is not as intuitive as methods R3.


%From the results of $T_{collision}$, it is reasonable to conclude that methods R1, R2 and R3 outperformed both method C and method H. This verified that the variable-scaling rate control is collision avoidance guaranteed when the risk of collision into account. Even though there is no obvious difference between method C and H, the survey results that no users picked method C as their first choice to fly the UAV near obstacles, indicates that the method H performs relatively better in the aspect of precision compared with method C. This result aligns well with our aim to introduce the user's input to the rate control, which is providing smaller commanded velocity to the UAV when the user is trying to control the position of the UAV more precisely.
